AIMO-2 Winning Solution: Building State-of-the-Art Mathematical Reasoning Models with OpenMathReasoning dataset

This paper presents our winning submission to the AI Mathematical Olympiad - Progress Prize 2 (AIMO-2) competition. Our recipe for building state-of-the-art mathematical reasoning models relies on three key pillars. First, we create a large-scale dataset comprising 540K unique high-quality math problems, including olympiad-level problems, and their 3.2M long-reasoning solutions. Second, we develop a novel method to integrate code execution with long reasoning models through iterative training, generation, and quality filtering, resulting in 1.7M high-quality Tool-Integrated Reasoning solutions. Third, we create a pipeline to train models to select the most promising solution from many candidates. We show that such generative solution selection (GenSelect) can significantly improve upon majority voting baseline. Combining these ideas, we train a series of models that achieve state-of-the-art results on mathematical reasoning benchmarks. To facilitate further research, we release our code, models, and the complete OpenMathReasoning dataset under a commercially permissive license.

==> tex/5_results.tex <==
% \section{Results}

% In this section we describe experimental results.
% In addition to \textbf{Comp-Math-24-25}, introduced in Section \ref{sec:comp-math-24-25}, we use Humanity's Last Exam dataset \cite{phan2025humanitysexam} subset, consisting of 975 text-only problems from "Math" category. We refer to it as \textbf{HLE-Math}.

% \subsection{Main results}

% Table \ref{tab:eval-results} highlights our core results. 

% \subsection{Analysis}

% \textbf{Controlling number of code executions:}

% As described in Section \ref{sec:tir-self-improvement}, after each code output we append a limit warning, that tells how many code executions model has remaining. Additionally, the initial prompt provides the information about the total number of code executions model available.

% \begin{table*}
% \centering
% \begin{tabular}{cccccc}
% \hline
% \textbf{Prompt CE} & \textbf{Limit warning} & \textbf{pass@1} & \textbf{maj@16} & \textbf{Num. of code blocks} & \textbf{Violated limit, \%} \\
% \hline
% 1  & & 52.93 & 69.53 & 1.0 & 5.4 \\
% 2  & & 57.40 & 70.31 & 1.6 & 1.7 \\
% 4  & With warning & 59.11 & 72.27 & 2.4 & 1.3 \\
% 8  & & 61.28 & 73.83 & 3.2 & 0.8 \\
% 16 & & 62.26 & 73.44 & 3.5 & 0.1 \\
% \hline
% 1  &  & 24.80 & 62.50 & 1.6 & 62.9 \\
% 2  &  & 44.12 & 69.92 & 1.9 & 29.4 \\
% 4  & Without warning & 54.96 & 71.09 & 2.3 & 7.8 \\
% 8  &  & 61.11 & 71.88 & 2.6 & 0.3 \\
% 16 &  & 61.33 & 73.83 & 2.6 & 0.1 \\
% \hline
% \end{tabular}
% \caption{OpenMath-Qwen-14B TIR performance results on Comp-Math-24-25 with different number of code executions given in the prompt, with and without code execution limit warning. \textit{Violated limit, \%} refers to the \% of generations that reached number of code executions specified in the prompt.}
% \label{tab:code_execution_metrics}
% \end{table*}
% % \begin{table*}
% %   \centering
% %   \begin{tabular}{ccccc}
% %     \hline
% %     \textbf{Prompt CE} & \textbf{pass@1} & \textbf{maj@16} & \textbf{Num. of code blocks} & \textbf{Num. violated limit, \%} \\
% %     \hline
% %     1 & 52.93 & 69.53 & 1.0 & 5.4 \\
% %     2 & 57.40 & 70.31 & 1.6 & 1.7 \\
% %     4 & 59.11 & 72.27 & 2.4 & 1.3 \\
% %     8 & 61.28 & 73.83 & 3.2 & 0.8 \\
% %     12  & 61.45 & 72.27 & 3.4 & 0.4 \\
% %     16  & 62.26 & 73.44 &  3.5 & 0.1 \\
% %     \hline
% %   \end{tabular}
% %   \caption{TIR performance results on Comp-Math-24-25 with different number of code executions given in the prompt. \textit{Num. violated limit, \%} refers to the \% of generations that reached number of code executions specified in the prompt.}
% %   \label{tab:code_execution_metrics}
% % \end{table*}


% \textbf{TIR degradation with pass@1:}

% We notice that despite being superior in majority@$k$ setting with TIR prompt, our models perform on par or even worse in pass@1, compared to CoT prompt. The results in Table \ref{tab:unfinished-solutions} suggest that the reason is that with the TIR prompt there are more unfinished solutions across all model sizes, with 1.5B clearly standing out. This is most likely due to differences between token lengths of TIR and CoT training data, with TIR data being on average X tokens vs. CoT Y tokens.


% \begin{table}
% \begin{tabular}{rcc}
% \hline
% Model & Prompt &  Unfinished Solutions, \% \\
% \hline
%  1.5B &    &  2.23 \\
%    7B &    CoT &  0.98 \\
%   14B &    &  1.13 \\
% \hline
%  1.5B &    & 40.31 \\
%    7B &    TIR &  6.45 \\
%   14B &    &   4.06 \\
% \hline
% \end{tabular}
% \caption{\% of unfinished solutions on Comp-Math-24-25 dataset. We generate 32k tokens and consider solution unfinished if it does not contain "$\backslash$boxed".}
% \label{tab:unfinished-solutions}
% \end{table}



